The H-index can be easily manipulated

We prove two complexity results about the H-index concerned with the Google scholar merge operation on one's scientific articles. The results show that, although it is hard to merge one's articles in an optimal way, it is easy to merge them in such a way that one's H-index increases. This suggests the need for an alternative scientific performance measure that is resistant to this type of manipulation.

==> ecmds.tex <==
%\newcommand{\myparpic}[1]{\parpic{{\raisebox{5mm}{#1}}}
%\vspace{-1mm}
%
%\NI} % use with argument like {\yn T}

\newcommand{\Searrow}{\begin{turn}{45}$\Downarrow$    \end{turn}}
\newcommand{\Swarrow}{\begin{turn}{135}$\Uparrow$   \end{turn}}
\newcommand{\myparpic}[1]{\parpic{{\darkgray{#1}}}}
\newcommand{\bfe}[1]{\begin{bfseries}\emph{#1}\end{bfseries}\index{#1}}
% \newcommand{\oldbfe}[1]{\begin{bfseries}\emph{#1}\end{bfseries}}
% \newcommand{\bfei}[1]{\begin{bfseries}\emph{#1}\end{bfseries}\index{#1}}
\newcommand{\inv}{\invisible}
%\newcommand{\IF}{\mbox{{\bf if}\ }}
%\newcommand{\FI}{\mbox{{\bf fi}}}
%\newcommand{\DO}{\mbox{{\bf do}\ }}
%\newcommand{\OD}{\mbox{{\bf od}}}
%\newcommand{\WHILE}{\mbox{{\bf while}\ }}
%\newcommand{\END}{\mbox{{\bf end}}}
%\newcommand{\THEN}{\mbox{\ {\bf then}\ }}
%\newcommand{\ELSE}{\mbox{\ {\bf else}\ }}
%\newcommand{\T}{\mbox{{\bf true}}}
%\newcommand{\F}{\mbox{{\bf false}}}
%\newcommand{\FAIL}{{\bf fail}}
\newcommand{\ES}{\mbox{$\emptyset$}}

\newcommand{\myla}{\mbox{$\:\leftarrow\:$}}
\newcommand{\myra}{\mbox{$\:\rightarrow\:$}}
\newcommand{\da}{\mbox{$\:\downarrow\:$}}
\newcommand{\ua}{\mbox{$\:\uparrow\:$}}
\newcommand{\La}{\mbox{$\:\Leftarrow\:$}}
\newcommand{\Ra}{\mbox{$\:\Rightarrow\:$}}
\newcommand{\tra}{\mbox{$\:\rightarrow^*\:$}}
\newcommand{\lra}{\mbox{$\:\leftrightarrow\:$}}
\newcommand{\bu}{\mbox{$\:\bullet \ \:$}}
\newcommand{\up}{\mbox{$\!\!\uparrow$}}

\newcommand{\A}{\mbox{$\ \wedge\ $}}
\newcommand{\bigA}{\mbox{$\bigwedge$}}
%\newcommand{\Or}{\mbox{$\ \vee\ $}}
\newcommand{\Orr}{\mbox{$\ \vee\ $}}
\newcommand{\U}{\mbox{$\:\cup\:$}}
\newcommand{\I}{\mbox{$\:\cap\:$}}
\newcommand{\sse}{\mbox{$\:\subseteq\:$}}

\newcommand{\po}{\mbox{$\ \sqsubseteq\ $}}
\newcommand{\spo}{\mbox{$\ \sqsubset\ $}}
\newcommand{\rpo}{\mbox{$\ \sqsupseteq\ $}}
\newcommand{\rspo}{\mbox{$\ \sqsupset\ $}}


\newcommand{\Mo}{\mbox{$\:\models\ $}}
\newcommand{\mtwo}{\mbox{$\:\models_{\it 2}\ $}}
\newcommand{\mthree}{\mbox{$\:\models_{\it 3}\ $}}
\newcommand{\Mf}{\mbox{$\:\models_{\it f\!air}\ $}}
\newcommand{\Mt}{\mbox{$\:\models_{\it tot}\ $}}
\newcommand{\Mwt}{\mbox{$\:\models_{\it wtot}\ $}}
\newcommand{\Mp}{\mbox{$\:\models_{\it part}\ $}}

\newcommand{\PR}{\mbox{$\vdash$}}

\newcommand{\fa}{\mbox{$\forall$}}
\newcommand{\te}{\mbox{$\exists$}}
\newcommand{\fai}{\mbox{$\stackrel{\infty}{\forall}$}}
\newcommand{\tei}{\mbox{$\stackrel{\infty}{\exists}$}}

\newcommand{\calA}{\mbox{$\cal A$}}
\newcommand{\calG}{\mbox{$\cal G$}}
\newcommand{\calB}{\mbox{$\cal B$}}

\newcommand{\LLn}{\mbox{$1,\ldots,n$}}
\newcommand{\LL}{\mbox{$\ldots$}}

\newcommand{\WP}{deterministic program}
\newcommand{\WPs}{deterministic programs}
\newcommand{\AW}{\mbox{{\bf await}-statement}}
\newcommand{\AWs}{\mbox{{\bf await}-statements}}

\newcommand{\IFP}{\mbox{$\IF B_1 \ra S_1 \Box \LL \Box B_n \ra S_n\ \FI$}}
\newcommand{\DOP}{\mbox{$\DO B_1 \ra S_1 \Box \LL \Box B_n \ra S_n\ \OD$}}
\newcommand{\DIP}{\mbox{$[S_1 \| \LL \| S_n]$}}
\newcommand{\IFPa}{\mbox{$\IF \Box^n_{i=1}\ B_i \ra S_i\ \FI$}}
\newcommand{\DOPa}{\mbox{$\DO \Box^n_{i=1}\ B_i \ra S_i\ \OD$}}

\newcommand{\MS}[1]{\mbox{${\cal M}[\![{#1}]\!]$}}
\newcommand{\newMS}[1]{\mbox{$[\![{#1}]\!]$}}
\newcommand{\newhat}[1]{\langle {#1} \rangle}
\newcommand{\M}[2]{\mbox{${\cal M}[\![{#1},{#2}]\!]$}}
\newcommand{\MF}[1]{\mbox{${\cal M}_{{\it f\!air}}[\![{#1}]\!]$}}
\newcommand{\MT}[1]{\mbox{${\cal M}_{{\it tot}}[\![{#1}]\!]$}}
\newcommand{\MP}[1]{\mbox{${\cal M}_{{\it part}}[\![{#1}]\!]$}}
\newcommand{\MWT}[1]{\mbox{${\cal M}_{{\it wtot}}[\![{#1}]\!]$}}
\newcommand{\NS}[1]{\mbox{${\cal N}[\![{#1}]\!]$}}

\newcommand{\ITE}[3]{\mbox{$\IF {#1} \THEN {#2} \ELSE {#3}\ \FI$}}
\newcommand{\IT}[2]{\mbox{$\IF {#1} \THEN {#2}\ \FI$}}
\newcommand{\WD}[1]{\mbox{$\WHILE {#1}\ \DO$}}
\newcommand{\WDD}[2]{\mbox{$\WHILE {#1}\ \DO {#2}\ \OD$}}
\newcommand{\W}[1]{\mbox{${\bf wait}\ {#1}$}}
\newcommand{\AT}[1]{\mbox{${\bf await}\ {#1}\ {\bf then}$}}
\newcommand{\ATE}[2]{\mbox{${\bf await}\ {#1} \THEN {#2}\ \END$}}
\newcommand{\ATOM}[1]{\mbox{$\langle {#1} \rangle$}}
\newcommand{\RU}[2]{\mbox{${\bf repeat}\ {#1}\ {\bf until}\ {#2}$}}

\newcommand{\TF}[1]{\mbox{$T_{{\it f\!air}}({#1})$}}
\newcommand{\TFn}{\mbox{$T_{{\it f\!air}}$}}

\newcommand{\HT}[3]{\mbox{$\{{#1}\}\ {#2}\ \{{#3}\}$}}

\newcommand{\sg}{{\mbox{$\sigma$}}}
\newcommand{\Sg}{{\mbox{$\Sigma$}}}
\newcommand{\om}{{\mbox{$\omega$}}}
\newcommand{\al}{{\mbox{$\alpha$}}}
\newcommand{\ba}{{\mbox{$\beta$}}}

\newcommand{\B}[1]{\mbox{$[\![{#1}]\!]$}}       % brackets
\newcommand{\C}[1]{\mbox{$\{{#1}\}$}}           % curly braces

\newcommand{\UPDATE}{\mbox{$U\!P\!D\!AT\!E$}}
\newcommand{\INIT}{\mbox{$I\!N\!IT$}}
\newcommand{\SCH}{\mbox{$SC\!H$}}
\newcommand{\FAIR}{\mbox{$F\!AI\!R$}}
\newcommand{\RORO}{\mbox{$RO\!RO$}}
\newcommand{\QUEUE}{\mbox{$QU\!EU\!E$}}
\newcommand{\INV}{\mbox{$IN\!V$}}
\newcommand{\VAR}{\mbox{\it Var}}
\newcommand{\unfold}{\mbox{\it unfold}}
\newcommand{\fold}{\mbox{\it fold}}
\newcommand{\ol}[1]{\mbox{$\overline{{#1}}$}}
\newcommand{\NI}{\noindent}
\newcommand{\HB}{\hfill{$\Box$}}
\newcommand{\VV}{\vspace{5 mm}}
\newcommand{\III}{\vspace{3 mm}}
\newcommand{\II}{\vspace{2 mm}}
\newcommand{\PP}{\mbox{$[S_1 \| \LL \| S_n]$}}

\newcommand{\X}[1]{\mbox{$\:\stackrel{{#1}}{\rightarrow}\:$}}
\newcommand{\lX}[1]{\mbox{$\:\stackrel{{#1}}{\longrightarrow}\:$}}

%\newcommand{\bold}[1]{{\bf #1}}  % for makeindex
%\newcommand{\see}[2]{{\it see\/} #1}  % for makeindex

%\newenvironment{myv}{\begin{verbatim} \small}{\normalsize \end{verbatim}} %for programs

\newenvironment{mydef}{\begin{boxitpara}{box 0.95 setgray fill}}{\end{boxitpara}}

%\newcommand{\error}{{\bf error}}
\newcommand{\vect}[1]{{\bf #1}}
\newcommand{\D}[1]{\mbox{$|[{#1}]|$}}           % |[ ]| braces
\newcommand{\hb}[1]{{\Theta_{#1}}}
\newcommand{\hi}{{\cal I}}
\newcommand{\ran}{\rangle}
\newcommand{\lan}{\langle}
\newcommand{\dom}{{\it Dom}}
\newcommand{\var}{{\it Var}}
\newcommand{\pred}{{\it pred}}
\newcommand{\sem}[1]{{\mbox{$[\![{#1}]\!]$}}}
\newcommand{\false}{{\it false}}
\newcommand{\true}{{\it true}}
\newtheorem{Property}{Property}[section]
\newcommand{\hsuno}{\hspace{ .5in}}
\newcommand{\vsuno}{\vspace{ .25in}}
\newcommand{\cons}{$\! \mid $}
\newcommand{\nil}{[\,]}
\newcommand{\restr}[1]{\! \mid \! {#1}} 
\newcommand{\range}{{\it Ran}}
\newcommand{\Range}{{\it Range}}
\newcommand{\PC}{\mbox{$\: \simeq \:$}}
\newcommand{\TC}{\mbox{$\: \simeq_t \:$}}
\newcommand{\IO}{\mbox{$\: \simeq_{i/o} \:$}}
\newcommand{\size}{{\rm size}}
\newcommand{\Der}[2]
        {\; |\stackrel{#1}{\!\!\!\longrightarrow _{#2}}\; }

\newcommand{\Sder}[2]
        {\; |\stackrel{#1}{\!\leadsto_{#2}}\; }

%\newcommand{\nat} { \mbox{\hspace{0.4ex}} {\rm N}
%                   \mbox{\hspace{-2.0ex}} {\rm I} \mbox{\hspace{0.8ex}}}
%
%\newcommand{\pif}{\leftarrow}
%\newcommand{\clause}[2]{#1 & \!\!\!\! \pif & \!\!\!\! #2} %\clause{head}{body}
%\newcommand{\comclause}[3]{\clause{#1}{#2}&\mbox{\% #3}}  %...{comment}
%
%\newenvironment{program}%                     % program with clauses numbered
%{\begin{eqnarray}\setcounter{equation}{1}}%   % C1,...Cn
%{\end{eqnarray}}
%\renewcommand{\theequation}{C\arabic{equation}}
%
%\newenvironment{ack}%
%{{\vspace{2ex}\par \noindent \bf
%\bf Acknowledgements.}}{\ignorespaces}
%
%\newcommand{\qed}{\hfill*$\quad\Box$}
%\newenvironment{Pf}{\par \noindent{\bf Proof.~}}{\qed }
%

\newcommand{\szkew}[1]{\relax \setbox0=\hbox{\kern -24pt $\displaystyle#1$\kern 0pt }%
%\advance\ht0 by 0pt %
%\advance\dp0 by -10pt %
\box0}
{\catcode`\@=11 \global\let\ifjusthvtest@=\iffalse}
%\definemorphism{dashto}\dashed\tip\notip

\newcommand{\iif}{\mbox{$\longrightarrow$}}
\newcommand{\longra}{\mbox{$\longrightarrow$}}
\newcommand{\Longra}{\mbox{$\Longrightarrow$}}
\newcommand{\res}[3]{\mbox{$#1\stackrel{\textstyle #2}{\Longra}#3$}}
\newcommand{\reso}[4]{\mbox{
$#1 \stackrel{#2}{\Longra}_{\hspace{-4mm}_{#3}} \hspace{2mm} #4$}}
\newcommand{\nextres}[2]{\mbox{$\stackrel{\textstyle #1}{\Longra}#2$}}
\newcommand{\preres}[2]{\mbox{$#1\stackrel{\textstyle #2}{\Longra}$}}
\newcommand{\Preres}[2]{\mbox{$#1\stackrel{\textstyle #2}{\longra}$}}

%just deleted old in 4 lines below and commented three lines below
\newcounter{oldmycaption}
\newcommand{\oldmycaption}[1]
{\begin{center}\addtocounter{oldmycaption}{1}
{{\bf Program \theoldmycaption} : #1}\end{center}} 

\newcommand{\mycite}[1]{\cite{#1}\glossary{#1}}

\newcommand{\mycaption}[1]
{\begin{center}{{\bf Program:} $#1$}
\index{#1} \end{center}} 

\newcommand{\ass}{{\cal A}}
\newcommand{\defi}{{\stackrel{\rm def}{=}}}

%\newcommand{\textbf}[1]{{\bf #1}}

% from art/at.tex

\newcommand{\Seq}[1]{{\bf #1}}
\newcommand{\BSeq}[2]{{{#1}_1},\ldots,{{#1}_{#2}}}
\newcommand{\OSeq}[2]{{{#1}_0},\ldots,{{#1}_\alpha},\ldots}
\newcommand{\Var}[1]{{\it Var}({#1})}
\newcommand{\FreeVar}[1]{{\it FreeVar}({#1})}
\newcommand{\Dom}[1]{{\it Dom}({#1})}
\newcommand{\Ran}[1]{{\it Ran}({#1})}
\newcommand{\Neg}{\neg}
\newcommand{\Fail}{{\it fail}}
\newcommand{\Success}{\Box}
\newcommand{\Flounder}{{\it flounder}}
%\newcommand{\Error}{{\it error}}
\newcommand{\Prune}{{\it prune}}
\newcommand{\cut}{\mbox{\it cut}}
% from art/at.tex

\newcommand{\p}[2]{\langle #1 \ ; \ #2 \rangle}

\newcommand{\ceiling}[1]{\lceil #1 \rceil}
\newcommand{\adjceiling}[1]{\left \lceil #1 \right \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\adjfloor}[1]{\left \lfloor #1 \right \rfloor}


%%%%%%%%%%% for color slides

\newcommand{\mytitle}[1]
{\begin{center}\begin{Sbox} {\bf #1}\end{Sbox}\shadowbox{\TheSbox}\end{center}}

\newcommand{\myctitle}[1]
{\textRed\begin{center}\begin{Sbox} {\bf #1}\end{Sbox}\shadowbox{\TheSbox}\end{center}\textBlack}

%\newcommand{\blue}[1]
%{\textBlue#1\textBlack}

%\newcommand{\red}[1]
%{\textRed#1\textBlack}

%\newcommand{\brown}[1]
%{\textBrown#1\textBlack}

%\newcommand{\bblue}[1]
%{\textBlue{\bf#1}\textBlack}

%\newcommand{\bred}[1]
%{\textRed{\bf#1}\textBlack}

%\newcommand{\bbrown}[1]
%{\textBrown{\bf#1}\textBlack}

%%%%%%%%%%% for color slides
